A Whole-Body Software Abstraction layer for Control Design of free-floating Mechanical Systems

In this paper, we propose a software abstraction layer to simplify the design and synthesis of whole-body controllers without making any preliminary assumptions on the control law to be implemented. The main advantage of the proposed library is the decoupling of the control software from implementation details, which are related to the robotic platform. Furthermore, the resulting code is more clean and concise than ad-hoc code, as it focuses only on the implementation of the control law. In addition, we present a reference implementation of the abstraction layer together with a Simulink interface to provide support to Model-Driven based development. We also show the implementation of a simple proportional-derivative plus gravity compensation control together with a more complex momentum-based bipedal balance controller.

==> tex/requisites.tex <==
%!TEX root = ../wbi.tex
\section{Requirements}

What are the requirements for this software?
They have already been introduced in the introduction but we can expand a bit here.



